Ready Policy One: World Building Through Active Learning

Model-Based Reinforcement Learning (MBRL) offers a promising direction for sample efficient learning, often achieving state of the art results for continuous control tasks. However, many existing MBRL methods rely on combining greedy policies with exploration heuristics, and even those which utilize principled exploration bonuses construct dual objectives in an ad hoc fashion. In this paper we introduce Ready Policy One (RP1), a framework that views MBRL as an active learning problem, where we aim to improve the world model in the fewest samples possible. RP1 achieves this by utilizing a hybrid objective function, which crucially adapts during optimization, allowing the algorithm to trade off reward v.s. exploration at different stages of learning. In addition, we introduce a principled mechanism to terminate sample collection once we have a rich enough trajectory batch to improve the model. We rigorously evaluate our method on a variety of continuous control tasks, and demonstrate statistically significant gains over existing approaches.

==> discussion.tex <==

\section{Discussion}

Here we want to emphasize that 1) our model is not the optimal model 2) our policy optimizer is not the best RL algorithm. This is crucial so we are not compared to SAC (or the latest Sergey paper which incrementally builds upon SAC). 

We can include an adaptive rollout length when training the policy in the model.

==> ideas.tex <==



\section{Ready Policy One: Sketch Ideas}

\begin{enumerate}
    \item \textbf{Active Learning on Policies}: Say we have a world model, or an ensemble of world models. Instead of deciding which \textit{state} to explore/visit, we can decide which \textit{policy} we want to evaluate in the true environment, by training multiple policies and deciding (somehow) which one is the most interesting. After one rollout, we re-fit the model(s) and repeat. (\textbf{Phil: So the Akiyama paper does something similar in that they have various candidate ``sampling" policies which are simply the same policy with increasing degrees of $\epsilon$-greediness (i.e., 10 policies, from 0.1-1 greedy); could flip this and turn it into a temperature for a policy-gradient method})
    \item \textbf{Active Learning on Action Subsets}: Say we have a world model, and we wish to decide an action to take next. Therefore we can utilise an n-step horizon, and sample subsets of possible actions (i.e., say $n=3$, therefore Left, Right, Left), run them through the world model, and then select the next action which maximises world model uncertainty given subsequent roll-out. Difficulty is how do we select these subsets (i.e., combinatoric explosion). (\textbf{Jack: As $n\rightarrow H$ where $H$ is the rollout horizon, this becomes 1 above}).
    \item \textbf{Adversarial World Models (lol)}: Train a policy which is rewarded based on how much uncertainty it can force from a world model; then use that policy to collect real world trajectories. 
    \item \textbf{Sample Collection Early Stopping}: Currently the outer loop to collect data for a MBRL agent's internal model is fixed at some arbitrary length (i.e., 30 trajectories). It should be possible to measure the `rolling' diversity of the trajectories acquired so far, and decide when to stop. This should increase sample efficiency by reducing redundancy.
    \item \textbf{Active Learning Acquisition Function}: We can take inspiration from Bayesian Optimization, notably predictive entropy search, and train policies that maximize the expected reduction in posterior uncertainty of the world model.
\end{enumerate}


==> related_work.tex <==

\section{Related Work}
\label{sec:related_work}




\jcom{this is the set of notes to use, when writing the related work section}

\subsection{Most Similar to our stuff}

\textbf{\href{https://www.sciencedirect.com/science/article/pii/S0893608010000031}{Efficient exploration through active learning for value function approximation in reinforcement learning}}
\begin{itemize}
    \item Old school (i.e., basis functions are used) RL using value function approximation error as a proxy for how to explore.
    \item Scene: We can easily collect data, but don't have access to their respective rewards. We can obtain rewards eventually, but this is costly (the example they use is a robot arm hitting a baseball; it's easy to keep swinging and collect sensor readouts of the arm, but hard to measure the actual flight of the ball, which is what the reward is a function of).
    \item We want to learn a value function robustly, i.e., have it generalise well. It turns out we can estimate the generalisation of any value function given a policy without actually having access to the underlying rewards.
    \item So the question is this; given $n$ candidate policies we can use to generate trajectories, which policy's trajectories should we actually label so as to perform value function approximation which generalises?
    \item Simple: 1) Collect trajectories with all $n$ policies; 2) Estimate each policy's generalisation error; 3) Collect more trajectories with the policy that has the lowest generalisation error and label those for use in value function estimation.
    \item Now we just shove the previous step into an outer loop, and keep iterating (i.e., \textbf{select best exploration policy}, label that policy's data with rewards, improve value function, improve policy with improved value function, repeat).
    \item The policies are generated by varying the amount of $\epsilon$-greediness (i.e., 10 policies going from slightly random to completely random).
\end{itemize}
\textbf{\href{https://arxiv.org/pdf/1906.04161.pdf}{Self-Supervised Exploration via Disagreement}}
\begin{itemize}
    \item Quite a simple idea (annoyingly): 1) Learn an ensemble of dynamics models 2) Train a policy 3) For each state $s_t$ set the reward $r_t$ equal to the variance of the model predicted states $\hat s_{t+1}$. They can do this in a `self-supervised' manner since they don't use the actual reward. They claim to be doing active learning, but have zero maths (even less than the Uber papers).
    \item  ``The  policy  objective in Equation (2) can  be generalized to the multi-step  horizon setup by recursively applying the forward predictor ... In this paper, we show differentiable exploration results for short horizon only and leave multi-step scenarios for future work."
    \item ``‘Pred-Error Variance’ is an alternative ablation where we train the agent to maximize the variance ofthe prediction error as opposed to the variance of model output itself." - Interestingly this does rather badly, but no discussion why.
\end{itemize}

\subsection{Exploration in RL}


\textbf{\href{https://arxiv.org/pdf/1910.01913.pdf}{If MaxEnt RL is the Answer, What is the Question?}}\\
\\
\textbf{\href{https://sites.google.com/view/erl-2019/related-work?authuser=0}{Exploration RL Workshop Related Work}}\\

\subsection{Model Based RL}

\textbf{\href{https://arxiv.org/pdf/1805.12114.pdf}{Deep Reinforcement Learning in a Handful of Trials using Probabilistic Dynamics Models}}
\begin{itemize}
    \item Build a Bayesian NN as the model, which can model both epistemic and aleotoric uncertainty. By being able to capture these, the subsequent planning can be done more effectively, since multi-modality and inherent stochasticity can be taken into account. They use model predictive control to select the next action.
    \item Instead of random shooting (i.e., uniform random sampling of actions), they fit a Gaussian over action spaces, which is updated w.r.t. the top K performing sequences ordered by return. This means over time more rewarding action sequences are chosen. This is called CEM.
    \item 
\end{itemize}
\textbf{\href{https://arxiv.org/pdf/1810.12162.pdf}{Model-Based Active Exploration}}
\begin{itemize}
    \item Seems that the active term isn't necessarily a reference to active learning, but rather to contrast with passive approaches which `happen' upon novel states, and aim to revisit those (i.e., Pathak's curiosity work). Some nice tricks to resolve issues of doing maths in continuous domains (i.e., Jensen-Renyi). I wonder if a single powerful Bayes net would be better than the ensemble? Since each net only receives a subset, so individually they don't really leverage the entire data (they probably tried this and it didn't so...).
\end{itemize}
\textbf{\href{https://arxiv.org/pdf/1811.04551.pdf}{Learning Latent Dynamics for Planning from Pixels}}\\
\textbf{\href{https://arxiv.org/pdf/1803.10122.pdf}{World Models}}
\begin{itemize}
    \item World Models does random exploration, which is fine in the context of these 2 simple environments, but not so for say Montezuma's revenge (i.e., we'll build a very myopic internal model). There is no discussion about partial observability here, but seems capable of coping with that; I'll need to dig further, but I think there could be scope for leveraging Bayesian approaches to deal with POMDP environments + exploration by leveraging such an internal model. Perhaps the uncertainty due to partial observability can be used to encourage environment resolving behaviour, thus building a stronger internal model for example, which can be used for simulations to `hallucinate' better.
\end{itemize}

\textbf{\href{http://mlg.eng.cam.ac.uk/pub/pdf/DeiRas11.pdf}{PILCO}}\\
\\
\textbf{\href{https://arxiv.org/pdf/1712.05556.pdf}{Safe Policy Search Using Gaussian Process Models}}\\
\\
\textbf{\href{http://www.cs.ox.ac.uk/people/yarin.gal/website/PDFs/DeepPILCO.pdf}{Improving  PILCO  with  Bayesian  Neural  Network  Dynamics  Models}}\\
\\
\textbf{\href{https://arxiv.org/pdf/1907.02057.pdf}{Benchmarking Model-Based Reinforcement Learning}}

\subsection{Active Learning}

\textbf{\href{https://oatml.cs.ox.ac.uk/publications/201912_KAJvAYGBatchBALD.html}{BatchBALD: Efficient and Diverse Batch Acquisition for Deep Bayesian Active Learning}}\\
\begin{itemize}
    \item Extends the \href{https://arxiv.org/abs/1112.5745}{BALD} approach to batches; the original BALD does not work for batches because it considers each point separately. BALD is an acquisition function that selects points based on the mutual information between model weights and subsequent predictions; a datum that is maximally informative basically says that learning its true class would therefore inform us maximally about the true weights. However the algorithm is not good for batches since it considers each data point independently, leading to non-diverse batches (i.e., only selecting the number 8 in MNIST). Instead BatchBALD selects the most informative SUBSET of data (using a heuristic to prevent combinatoric explosion) which means higher entropy of classes in the batches.
    \item Overall framework seems to be as follows: a) have some unlabelled data; b) have some acquisition function we evaluate over unlabelled data to maximise something; c) have some oracle/expert which provides us labelled data upon request; d) you `win' when you minimse the number of times the oracle/expert is queried for a given level of accuracy (i.e., 90\% on MNIST)
    \item The above is framed in a supervised learning manner, need to reframe in an RL context.
\end{itemize}


